Sampling-based Fast Gradient Rescaling Method for Highly Transferable Adversarial Attacks

Deep neural networks are known to be vulnerable to adversarial examples crafted by adding human-imperceptible perturbations to the benign input. After achieving nearly 100% attack success rates in white-box setting, more focus is shifted to black-box attacks, of which the transferability of adversarial examples has gained significant attention. In either case, the common gradient-based methods generally use the sign function to generate perturbations on the gradient update, that offers a roughly correct direction and has gained great success. But little work pays attention to its possible limitation. In this work, we observe that the deviation between the original gradient and the generated noise may lead to inaccurate gradient update estimation and suboptimal solutions for adversarial transferability. To this end, we propose a Sampling-based Fast Gradient Rescaling Method (S-FGRM). Specifically, we use data rescaling to substitute the sign function without extra computational cost. We further propose a Depth First Sampling method to eliminate the fluctuation of rescaling and stabilize the gradient update. Our method could be used in any gradient-based attacks and is extensible to be integrated with various input transformation or ensemble methods to further improve the adversarial transferability. Extensive experiments on the standard ImageNet dataset show that our method could significantly boost the transferability of gradient-based attacks and outperform the state-of-the-art baselines.

==> 025DefenseRW.tex <==
\subsection{Adversarial Defenses}
%% Adversarial training and Input modification and certified defense

On the other hand, many adversarial defense methods have been proposed to mitigate the threat of adversarial examples. 

\subsubsection{Adversarial Training}
A natural idea for improving the model robustness is to generate adversarial examples by attacking the model and then use the crafted examples to optimize the model. Goodfellow~\etal~\citeyearpar{goodfellow2014explaining} discover that adding adversarial examples for model training could improve the model robustness. More recently, Madry~\etal~\citeyearpar{madry2018towards} showed that the adversarial training process could be formulated as solving a minimax optimization problem. Tramèr~\etal~\citeyearpar{tramer2018ensemble} propose ensemble adversarial training, which augments the training data with perturbations generated by several models. Recently, Gong~\etal~\citeyearpar{gong2021maxup} propose a lightweight variant of adversarial training called MaxUp, which is simpler and faster. 


\subsubsection{Data or Feature Processing}
In addition to adversarial training, input transformation and feature preprocessing are also proposed to defend against  adversarial attacks. 
Xie~\etal~\citeyearpar{xie2018mitigating} add a randomization layer with random resizing and padding to models to mitigate the adversarial effects, while Xu~\etal~\citeyearpar{xu2018feature} reduce the search space of adversarial perturbation by feature squeeze, and Guo~\etal~\cite{guo2017countering} apply image transformations such as JPEG compression and image quilting to training the models. 
Liao~\etal~\citeyearpar{liao2018defense} propose a high-level representation guided denoiser (HGD) to improve the robustness. 
Liu~\etal~\citeyearpar{liu2019feature} propose a JPEG-based defensive compression framework called feature distillation (FD) to guarantee the defense efficiency and classification accuracy on benign data. Jia~\etal~\citeyearpar{jia2019comdefend} propose an end-to-end image compression model dubbed ComDefend to improve the robustness efficiently. Naseer~\etal~\citeyearpar{naseer2020self} combine adversarial training with input processing and train a purified model called Neural Representation Purifier (NPR).

\subsubsection{Certified Robustness}
Despite being robust under strong attacks, models obtained by adversarial training still need verified error guarantees and certified safety. So provable adversarial defense provides a method to certify the robustness of learned neural networks under unknown attacks. Wong~\etal~\citeyearpar{wangprovable2018} propose linear relaxations of neural networks to give an upper bound of the inner max of adversarial training optimization. However, the bound propagation process of a convex adversarial polytope is too expensive. Gowal~\etal~\citeyearpar{Gowalibp2018} propose Interval Bound Propagation (IBP) to use a straightforward rule to compute the pre-activation outer bounds for each layer of the network. Zhang~\etal~\citeyearpar{zhang2021towards} propose a $l_\infty$-dist net, which is a 1-Lipschitz function, and the bound can be easily found in only a forward pass to resist $l_\infty$ perturbation.



==> fig/evaluationrescale.tex <==
\begin{figure}[htbp]
    \centering
    \begin{minipage}[c]{0.23\textwidth}
        \centering
        %\vspace{1.05cm}
        \includegraphics[width=0.85\linewidth]%[width=0.75\linewidth]
        {fig/samplecoef.pdf}
        %\subcaption{(a)SMI-FGRM}
        \label{subfig:cmpFGSM}
    \end{minipage}
    %\hspace{0.05cm}
    \begin{minipage}[c]{0.23\textwidth}%{0.45\textwidth}
        \centering
        \includegraphics[width=0.85\linewidth]{fig/cmpS2M.pdf}
        %\subcaption{(b)SNI-FGRM}
        \label{subfig:cmpS2M}
    \end{minipage}
    \caption{The attack success rates (\%) on six models with adversarial examples generated by Inc-v3 for various scale factors of $c$. The dashed lines represent the vanilla method of I-FGSM on the left and I-FGS$^2$M with their best settubg of $k = 64$ for Staircase on the right.}
    \label{fig:srescale}
    % \vspace{-0.5em}
\end{figure}

==> tab/C_I.tex <==
\begin{table*}[ht]
  \centering
    \caption{Attack success rates (\%) of adversarial attacks on seven models in the single model setting with different parameter $c$. The adversarial examples are crafted on Inc-v3, Inc-v4, IncRes-v2, and Res-101 respectively. * indicates the white-box model.}
  \label{tab:C_I}
    \resizebox{0.88\textwidth}{!}{
    \begin{tabular}{ l|l||c c c c c c c }
    \toprule
    Model & Attack & Inc-v3 & Inc-v4 & IncRes-v2 & Res-101 & Inc-v3$_{ens3}$ & Inc-v3$_{ens4}$ & IncRes-v2$_{ens}$ \\
    \midrule
    \multirow{6}{*}{Inc-v3} 
    & I-FGSM &100.0*&21.0&19.1&15.8&5.1&5.0&2.3 \\
    & I-FGS$^2$M &100.0*&34.2&31.0&25.5&\textbf{9.5}&9.6&4.0 \\
    \cmidrule{2-9}
    & I-FGRM(2) &100.0*&30.5&28.8&22.4&7.3&7.8&3.6\\
    & I-FGRM(3) &100.0*&38.1&35.9&30.4&8.9&\textbf{9.9}&4.2\\
    & I-FGRM(4) &100.0*&\textbf{41.3}&\textbf{37.9}&\textbf{30.5}&8.8&9.3&4.1\\
    & I-FGRM(5) &100.0*&40.6&37.4&29.8&7.6&9.6&\textbf{4.6}\\
    \midrule
    \multirow{6}{*}{Inc-v4} 
    & I-FGSM &31.6&99.9*&20.0&20.0&5.4&6.1&3.3\\
    & I-FGS$^2$M &45.2&100.0*&32.1&28.4&10.8&9.7&5.0\\
    \cmidrule{2-9}
    & I-FGRM(2) &41.4&99.9*&29.4&27.1&8.1&8.4&4.7\\
    & I-FGRM(3) &49.6&99.9*&\textbf{38.4}&32.5&\textbf{11.3}&9.3&\textbf{6.0}\\
    & I-FGRM(4) &\textbf{50.9}&100.0*&38.0&\textbf{34.8}&9.2&\textbf{9.9}&5.3\\
    & I-FGRM(5) &49.4&100.0*&35.7&31.6&9.3&8.0&5.0\\
    \midrule
    \multirow{6}{*}{IncRes-v2} 
    & I-FGSM &33.4&25.1&98.2*&21.0&7.7&6.4&4.5\\
    & I-FGS$^2$M &43.8&36.7&98.6*&30.4&\textbf{14.4}&\textbf{11.0}&\textbf{8.1}\\
    \cmidrule{2-9}
    & I-FGRM(2) &43.3&34.4&98.7*&27.5&11.5&9.6&6.7\\
    & I-FGRM(3) &50.9&40.7&98.8*&32.1&13.0&\textbf{11.0}&7.3\\
    & I-FGRM(4) &\textbf{52.3}&41.4&98.9*&\textbf{33.6}&11.6&9.8&7.4\\
    & I-FGRM(5) &52.2&\textbf{41.6}&99.2*&33.3&10.0&9.2&6.2\\
    \midrule
    \multirow{5}{*}{Res-101} 
    & I-FGSM &31.2&25.2&21.9&99.3*&7.9&7.6&5.1\\
    & I-FGS$^2$M &44.9&37.5&34.6&99.4*&\textbf{17.7}&\textbf{15.2}&\textbf{10.0}\\
    \cmidrule{2-9}
    & I-FGRM(2) &40.6&35.7&33.6&99.3*&14.9&12.7&7.2\\
    & I-FGRM(3) &51.7&45.8&41.3&99.4*&17.5&14.1&8.8\\
    & I-FGRM(4) &53.0&\textbf{49.0}&45.5&99.4*&17.2&14.0&8.4\\
    & I-FGRM(5) &\textbf{53.6}&48.3&\textbf{45.8}&99.4*&15.7&12.7&7.1\\
    \bottomrule
    \end{tabular}
    }

    %\vspace{-4mm}
\end{table*}

==> tab/C_MI.tex <==
\begin{table*}[ht]
  \centering
    \caption{Attack success rates (\%) of adversarial attacks on seven models in the single model setting with momentum as well as different parameter $c$ . The adversarial examples are crafted on Inc-v3, Inc-v4, IncRes-v2, and Res-101 respectively. * indicates the white-box model.}
  \label{tab:C_MI}
    \resizebox{0.88\textwidth}{!}{
    \begin{tabular}{ l|l||c c c c c c c }
    \toprule
    Model & Attack & Inc-v3 & Inc-v4 & IncRes-v2 & Res-101 & Inc-v3$_{ens3}$ & Inc-v3$_{ens4}$ & IncRes-v2$_{ens}$ \\
    \midrule
    \multirow{6}{*}{Inc-v3} 
    & MI-FGSM &100.0*&43.6&42.5&36.1&13.2&\textbf{13.0}&6.6\\
    & MI-FGS$^2$M &100.0*&48.2&45.7&40.2&13.3&12.6&6.1\\
    \cmidrule{2-9}
    & MI-FGRM(2) &100.0*&46.3&45.5&38.6&\textbf{14.1}&12.4&\textbf{7.0}\\
    & MI-FGRM(3) &100.0*&48.4&47.2&39.3&11.3&12.0&5.7\\
    & MI-FGRM(4) &100.0*&48.8&48.1&39.3&11.6&11.4&5.3\\
    & MI-FGRM(5) &100.0*&\textbf{49.8}&\textbf{49.7}&\textbf{40.5}&10.0&10.5&4.9\\
    \midrule
    \multirow{6}{*}{Inc-v4} 
    & MI-FGSM &56.2&99.9*&46.2&41.2&16.7&\textbf{15.3}&7.5\\
    & MI-FGS$^2$M &60.4&100.0*&49.4&43.3&17.6&\textbf{15.3}&7.0\\
    \cmidrule{2-9}
    & MI-FGRM(2) &57.2&99.9*&48.4&44.2&\textbf{18.5}&14.7&\textbf{7.9}\\
    & MI-FGRM(3) &59.0&100.0*&\textbf{51.1}&43.1&14.7&12.8&5.9\\
    & MI-FGRM(4) &61.8&100.0*&50.3&\textbf{44.9}&13.0&13.0&5.6\\
    & MI-FGRM(5) &\textbf{62.1}&100.0*&50.8&44.4&12.4&11.3&5.8\\
    \midrule
    \multirow{6}{*}{IncRes-v2} 
    & MI-FGSM &59.9&48.4&97.8*&44.9&\textbf{22.9}&16.5&11.5\\
    & MI-FGS$^2$M &62.8&53.1&98.3*&\textbf{47.8}&\textbf{22.9}&\textbf{17.9}&11.3\\
    \cmidrule{2-9}
    & MI-FGRM(2) &61.6&52.9&98.6*&44.7&21.9&16.8&\textbf{11.8}\\
    & MI-FGRM(3) &\textbf{63.5}&\textbf{55.0}&98.2*&46.4&17.3&14.8&8.6\\
    & MI-FGRM(4) &63.3&54.4&99.1*&45.8&15.9&13.2&8.2\\
    & MI-FGRM(5) &63.2&51.2&98.9*&44.8&14.4&12.2&7.9\\
    \midrule
    \multirow{5}{*}{Res-101} 
    & MI-FGSM &57.6&52.6&49.7&99.2*&24.5&21.5&13.0\\
    & MI-FGS$^2$M &59.3&53.1&52.8&99.3*&\textbf{26.0}&\textbf{23.3}&13.0\\
    \cmidrule{2-9}
    & MI-FGRM(2) &59.7&52.4&51.8&99.3*&\textbf{26.0}&22.8&\textbf{13.6}\\
    & MI-FGRM(3) &61.8&55.3&\textbf{54.0}&99.3*&23.2&20.5&10.8\\
    & MI-FGRM(4) &\textbf{63.8}&55.5&53.5&99.3*&20.5&18.7&10.2\\
    & MI-FGRM(5) &62.2&\textbf{57.0}&\textbf{54.0}&99.3*&19.4&17.5&7.8\\
    \bottomrule
    \end{tabular}
    }

    %\vspace{-4mm}
\end{table*}
